Will You Dance To The Challenge? Predicting User Participation of TikTok Challenges

TikTok is a popular new social media, where users express themselves through short video clips. A common form of interaction on the platform is participating in "challenges", which are songs and dances for users to iterate upon. Challenge contagion can be measured through replication reach, i.e., users uploading videos of their participation in the challenges. The uniqueness of the TikTok platform where both challenge content and user preferences are evolving requires the combination of challenge and user representation. This paper investigates social contagion of TikTok challenges through predicting a user's participation. We propose a novel deep learning model, deepChallenger, to learn and combine latent user and challenge representations from past videos to perform this user-challenge prediction task. We collect a dataset of over 7,000 videos from 12 trending challenges on the ForYouPage, the app's landing page, and over 10,000 videos from 1303 users. Extensive experiments are conducted and the results show that our proposed deepChallenger (F1=0.494) outperforms baselines (F1=0.188) in the prediction task.

==> abalation.tex <==
\begin{table}[!ht]
\caption{Full results of performance on challenge and user representation proxy tasks, and user-challenge participation prediction task }
\label{tab:full}
\begin{center}
% \small
%  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|ccc}
\hline
\textbf{Model} & \textbf{Macro-Prec} & \textbf{Macro-Rec} & \textbf{Macro-F1} \\ \hline \hline
\multicolumn{4}{l}{\textbf{Challenge Representation Proxy Task}} \\ \hline
Video (VGG) & 0.248 & 0.186 & 0.153 \\ 
Video (VGG) + Attention & 0.246 & 0.218 & 0.193 \\ 
Video (VGG) + Text (BERT) & \textbf{0.660} & \textbf{0.563} & \textbf{0.494} \\ 
Video (VGG) + Video numeric & 0.297 & 0.439 & 0.335 \\
Video (ResNet-50) & 0.257 & 0.174 & 0.125 \\ 
Video (ResNet-50) + Attention & 0.276 & 0.227 & 0.207 \\ 
Video (ResNet-50) + Text (BERT) & 0.583 & 0.486 & 0.385 \\ 
Video (ResNet-50) + Video numeric & 0.321 & 0.372 & 0.236 \\ 
\hline
\multicolumn{4}{l}{\textbf{User Representation Proxy Task}} \\ \hline
Video (VGG) & 0.163 & 0.558 & 0.163 \\ 
Video (VGG) + Attention & 0.167 & 0.600 & 0.166 \\ 
Video (VGG) + Text (BERT) & 0.186 & 0.749 & 0.188 \\ 
Video (ResNet-50) & 0.194 & 0.725 & 0.195 \\ 
Video (ResNet-50) + Attention & 0.191 & 0.723 & 0.191 \\ 
Video (ResNet-50) + Text (BERT) & \textbf{0.197} & \textbf{0.733} & \textbf{0.197} \\ 
\hline
\multicolumn{4}{l}{\textbf{User-Challenge Participation Task}} \\ \hline
Challenge Representation + User Representation & \textbf{0.4940} & \textbf{0.9330} & \textbf{0.4944} \\
\hline
\end{tabular}
%}
\end{center}
\end{table}

==> baselineresults.tex <==
\begin{table}[!ht]
\caption{Baseline Results}
\label{tab:baselineresults}
\begin{center}
% \small
%  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|ccc}
\hline
\textbf{Model} & \textbf{Macro-Prec} & \textbf{Macro-Rec} & \textbf{Macro-F1} \\ \hline \hline
Video (VGG) & 0.017 & 0.200 & 0.083 \\ 
Video (VGG) + Text (BERT) & 0.188 & 0.750 & \textbf{0.188} \\ 
Video (VGG) + Attention & 0.174 & 0.542 & 0.174 \\ 
Video (ResNet-50) & 0.050 & 0.059 & 0.050 \\ 
Video (ResNet-50) + Attention & 0.150 & 0.558 & 0.163 \\
Video (ResNet-50) + Text (BERT) & 0.186 & 0.750 & \textbf{0.188} \\ 
\hline
\end{tabular}
%}
\end{center}
\end{table}

==> challengetable.tex <==
\begin{table*}[t]
\caption{Statistics of the collected Challenge dataset}
\label{tab:challengestats}
\begin{center}
 \small
%  \resizebox{0.8\textwidth}{!}{
\begin{tabular}{p{3.25cm}|p{7.25cm}cc }
\hline

\textbf{Challenge} & \textbf{Description} & \textbf{\#videos} & \textbf{\#views}\\ \hline \hline
\#attentionchallenge & Shows off home gymnastics moves to the song Attention by Todrick Hall & 882 & 509,826,200\\ \hline
\#blindinglightschallenge & Three family members perform a dance together during quarantine & 946 & 1,524,481,619 \\ \hline
\#100wayschallenge & Retakes the pop idol Jackson Wang's dance to promote 100 ways to stay connected in South Korea & 999 & 7457,933 \\ \hline
\#BoredInTheHouse & Features daily life in isolation & 976 & 2,457,902,575 \\ \hline
\#anysongchallenge & Retakes the opening of the song Any Song by Zica' & 925 & 470,628,233 \\ \hline
\#karenchallenge & Complaining about an annoying, interfering adult & 1000 & 81,015,218 \\ \hline
\#Cannibalchallenge & Retakes dance moves of Ke\$ha's Cannibal at home & 907 & 866,017,300 \\ \hline 
\#renegadechallenge & Dance to a section of Lottery by K Camp & 1000 & 1,287,548,700 \\ \hline
\#washyourhandschallenge & Dance to promote washing hands & 225 & 945,039,700 \\ \hline
\#ghencovychallenge & Vietnamese dance to promote washing hands & 299 &  45,595,111 \\ \hline 
\#godaddygo & Dance to a section of Go Daddy Go by Dj Shawny & 284 &  347,123,549\\ \hline
\#papertowelchallenge & Reveal a secret message  when one puts a paper towel in water& 498 & 1,008,295,400 \\ \hline




%\textbf{Challenge} & \textbf{Description} & \textbf{\#videos} & \textbf{\#likes} & \textbf{\#shares} & \textbf{\#comments} & \textbf{\#views}\\ \hline \hline
%\#attentionchallenge & \begin{tabular}[c]{@{}c@{}}Shows off home gymnastics \\moves to the song Attention \\by Todrick Hall \end{tabular} & 882 & 64,179,524 & 2460263 & 647366 & 509826200\\ \hline
%\#blindinglightschallenge & \begin{tabular}[c]{@{}c@{}}Three family members perform\\ a dance together during quarantine \end{tabular} & 946 & 218603925 & 6090533 & 1409776 & 1524481619 \\ \hline
%\#100wayschallenge & \begin{tabular}[c]{@{}c@{}} Retakes the pop idol \\Jackson Wang's dance to promote \\100 ways to stay connected \\in South Korea \end{tabular} & 999 & 1115328 & 12547 & 14626 & 7457933 \\ \hline
%\#BoredInTheHouse & Features daily life in isolation & 976 & 256802523& 7350339 & 2023104 & 2457902575 \\ \hline
%\#anysongchallenge & \begin{tabular}[c]{@{}c@{}}Retakes the opening of \\ the song Any Song by Zica'  \end{tabular} & 925 & 33198592& 752221 & 281838 & 470628233 \\ \hline
%\#karenchallenge & \begin{tabular}[c]{@{}c@{}}Complaining about an annoying,\\ interfering adult \end{tabular} & 1000 & 19568377& 144764 & 120680 & 81015218 \\ \hline
%\#Cannibalchallenge & \begin{tabular}[c]{@{}c@{}}Retakes dance moves of \\Ke\$ha's Cannibal at home \end{tabular} & 907 & 92002397 & 1171411 & 774308 & 866017300 \\ \hline 
%\#renegadechallenge & \begin{tabular}[c]{@{}c@{}} Dance to a section of \\ Lottery by K Camp \end{tabular}& 1000 & 175559100 & 5681881 & 2086317 & 1287548700 \\ \hline
%\#washyourhandschallenge & \begin{tabular}[c]{@{}c@{}} Dance to promote \\ washing hands \end{tabular} & 225 & 108850600 & 2641012 & 739027 & 945039700 \\ \hline
%\#ghencovychallenge & \begin{tabular}[c]{@{}c@{}} Vietnamese dance to \\ promote washing hands \end{tabular} & 299 & 2849183 & 57198 & 2226 & 45595111 \\ \hline 
%\#godaddygo & \begin{tabular}[c]{@{}c@{}} Dance to a section of \\ Go Daddy Go by Dj Shawny \end{tabular}& 284 & 48146528 & 660431 & 483701 & 347123549\\ \hline
%\#papertowelchallenge & \begin{tabular}[c]{@{}c@{}} Reveal a secret message \\ when one puts a paper towel \\ in water  \end{tabular}& 498 & 132882837 & 3586489 & 145714 & 1008295400 \\ \hline


\end{tabular}

% }
\end{center}
\end{table*}
